Machine Learning Meets Quantitative Planning: Enabling Self-Adaptation in Autonomous Robots

Modern cyber-physical systems (e.g., robotics systems) are typically composed of physical and software components, the characteristics of which are likely to change over time. Assumptions about parts of the system made at design time may not hold at run time, especially when a system is deployed for long periods (e.g., over decades). Self-adaptation is designed to find reconfigurations of systems to handle such run-time inconsistencies. Planners can be used to find and enact optimal reconfigurations in such an evolving context. However, for systems that are highly configurable, such planning becomes intractable due to the size of the adaptation space. To overcome this challenge, in this paper we explore an approach that (a) uses machine learning to find Pareto-optimal configurations without needing to explore every configuration and (b) restricts the search space to such configurations to make planning tractable. We explore this in the context of robot missions that need to consider task timeliness and energy consumption. An independent evaluation shows that our approach results in high-quality adaptation plans in uncertain and adversarial environments.

==> sections/discussion.tex <==
%!TEX root = ../paper.tex
\section{Lessons Learned and Discussion}
\label{sec:discussion}

% I plan to discuss some lessons learned via our discussion debugging the planner through github. I think that is useful for SEMAS.


To the best of our knowledge, this work is the first contribution in the SEAMS community where evaluation was conducted by a third party, so we aim to share our experience during this evaluation process by discussing the pros and cons of it.

We start by explaining few decisions that helped us to facilitate the process:

During integration we used GitHub Enterprise as the coordination mechanism between our team and Lincoln Laboratory. We committed the code directly related to the evaluation to a private repository on GitHub. All coordination were done via the built-in issue tracker of the repository. Over a period of one year from problem definition, integration period and delivery of the code for test, over 120 issues were created from as low as 1 comment to 120 comments per issue. We used the issue tracking for not only allowing the evaluator to report any issues with respect to the system, but also if we had faced any issue with respect to the testing infrastructure or API definition. 

To enable the third party evaluation, we defined strategies, guidelines, and heuristics for designing representative tests that exercise adaptations. More specifically, we provide explanations for the selection of parameters, with knowledge of any interdependence on each, and the selection of their values for constructing representative tests.




This work was conducted as a part of the DARPA BRASS program\footnote{Building Resource Adaptive Software Systems program (BRASS): \url{https://www.darpa.mil/program/building-resource-adaptive-software-systems}}.
The independent evaluation supports the BRASS program goals by providing measures related to each of program goals: (i) discovering system intents, (ii) realizing the intents, (iii) recovering the intents. While we produced a system that could be tested (SUT), Lincoln Laboratory designed a test harness (TH) that could choose and evaluate particular test cases.

The integration with the test infrastructure was conducted in the following phases: 
\begin{itemize}
\item \textbf{Risk Reduction 1}: The API enabling integration between the test harness (evaluator side) and SUT was designed and stubs implemented that showed that the API worked as expected. The goal is to ensure mutual understanding of the interfaced between Lincoln Laboratory and system we designed. After this stage, the API was deemed stable and only minor changes were allowed afterwards.
\item \textbf{Risk Reduction 2}: A functional SUT integrated with the interface API and interaction code tested in the previous Risk Reduction. The goal of Risk Reduction 2 was to demonstrate the automated execution of each Challenge Problem running on the evaluation infrastructure which was used in the final testing.
\item \textbf{Risk Reduction 3}: A simulated evaluation is conducted wherein the SUT was tested as it would be in final testing, but in fewer and perhaps simplified cases. In addition to ensuring that a test could be run from start to end, Lincoln Laboratory also evaluated each test  to ensure that problems would not be encountered during the final evaluation process. All test verdicts and outputs should be representative of anticipated system operation. Also the tests in the stage were conducted in the same environment as the final evaluation, \emph{i.e.}, Amazon Cloud.
\item \textbf{Code Freeze}: This final stage was to deliver the code as well as environment for running the code so that it could be evaluated. 
\item \textbf{Test Execution}: Lincoln Laboratory ran tests based on our guidelines about the possible values each testing option can take: (i) number of tasks in a mission, (ii) power model, (iii) learning budget, (iv) number of obstacle placement, (v) number of battery perturbations.
\end{itemize}



% \BS{While this is useful information, I am not sure what the point of it is for this paper. We could consider removing it if we need space, or summarizing it with lessons learned about independent evaluation in a much shorter way.}


% Reproducibility

% Environment code all available

% Experience during Integration and Delivery

% Integration of model learning with Rainbow and planning, the mismatch and discussions

% Integration with test harness and working with an independent evaluator

% Experience during running tests


% \subsubsection*{Limitations}

